On Fairness and Stability in Two-Sided Matchings

There are growing concerns that algorithms, which increasingly make or influence important decisions pertaining to individuals, might produce outcomes that discriminate against protected groups. We study such fairness concerns in the context of a two-sided market, where there are two sets of agents, and each agent has preferences over the other set. The goal is producing a matching between the sets. This setting has been the focus of a rich body of work. The seminal work of Gale and Shapley formulated a stability desideratum, and showed that a stable matching always exists and can be found efficiently. We study this question through the lens of metric-based fairness notions (Dwork et al., Kim et al.). We formulate appropriate definitions of fairness and stability in the presence of a similarity metric, and ask: does a fair and stable matching always exist? Can such a matching be found in polynomial time? Our contributions are as follows: (1) Composition failures for classical algorithms: We show that composing the Gale-Shapley algorithm with fair hospital preferences can produce blatantly unfair outcomes. (2) New algorithms for finding fair and stable matchings: Our main technical contributions are efficient new algorithms for finding fair and stable matchings when: (i) the hospitals' preferences are fair, and (ii) the fairness metric satisfies a strong "proto-metric" condition: the distance between every two doctors is either zero or one. In particular, these algorithms also show that, in this setting, fairness and stability are compatible. (3) Barriers for finding fair and stable matchings in the general case: We show that if the hospital preferences can be unfair, or if the metric fails to satisfy the proto-metric condition, then no algorithm in a natural class can find a fair and stable matching. The natural class includes the classical Gale-Shapley algorithms and our new algorithms.

==> global_stability.tex <==
\section{Global stability}
In this section we show an algorithm that for proto-metric and strict individually fair preferences of the hospitals outputs an allocation which is PIIF and globally stable.

\subsection{Algorithm for Fair and Globally Stable Allocations}
We denote by $\mathcal{C}$ the set of all clusters in $\D$ and for every cluster $C \in \mathcal{C}$, we denote by $U(C)$ the uniform distribution over doctors in $C$.

In the algorithm below we define the set $\mathcal{S}$ to be a set of pairs of hospitals and clusters, we define ${\H}_{pool}$ to be the set of hospitals that are not a part of a pair in $\mathcal{S}$. Then we define the allocation $\pi(\mathcal{S})$ to be the allocation where in the first step, for every pair $(h, C) \in \mathcal{S}$, $h$ is matched to a doctor sampled from $U(C)$. For all the doctors that were not sampled in the first step and the hospitals in ${\H}_{pool}$, an allocation is chosen uniformly at random.

\begin{algorithm}[H]
\caption{Algorithm for Global Stability}
\label{alg:global_stability}
\begin{algorithmic}[1]
    \STATE ${\H}_{pool} \leftarrow \H, \mathcal{S} \leftarrow \set{}$.
    \WHILE{$\exists h \in {\H}_{pool}, C \in \mathcal{C}$ s.t. $U(C)$ and $h$ are a blocking allocation for $\pi(\mathcal{S})$}
        \STATE ${\H}_{pool} \leftarrow {\H}_{pool} \backslash \set{h}$.
        \STATE $\mathcal{S} \leftarrow \mathcal{S} \cup \set{(h, C)}$.
    \ENDWHILE
    \RETURN $\pi(\mathcal{S})$.
\end{algorithmic}
\end{algorithm}

\begin{lemma}
The output of \cref{alg:global_stability} is PIIF.
\end{lemma}
\begin{proof}
We start with the uniform distribution and then change the allocation per cluster.
Thus, for every $i_1,i_2$ in the same cluster $\pi(i_1) = \pi(i_2)$.
\end{proof}

\begin{lemma}
\label{lemma:alg_glob_term}
Algorithm \ref{alg:global_stability} stops after $O(|\mathcal{C}|)$ rounds.
\end{lemma}
\begin{proof}
Fix a cluster $C \in \mathcal{C}$, we claim that $C$ can participate at at most one blocking allocation during the run.
Assume for contradiction that the cluster $C$ participates in two blocking allocation with hospitals $h_1, h_2 \in \H$. Assume without loss of generality that at the first time that the algorithm finds a blocking allocation with $C$, it is with $h_1$.
Thus, when the blocking allocation with $h_1$ is found, $h_2$ is in $\H_{pool}$, i.e. $h_2$ is in the support of all the doctors in $C$. By the definition of blocking allocations, this implies that $\forall i \in C:h_1 \succ_i h_2$.

When the algorithm finds the blocking allocation with $h_2$, $h_1$ is in the support of the allocation of every doctor in $C$. We showed that $\forall i \in C:h_1 \succ_i h_2$ and this is a contradiction to the assumption that $h_2$ and $U(C)$ are a blocking allocation.

Thus, after $O(|\C|)$ iterations the algorithm must terminate.

\end{proof}

\begin{lemma}
The output of the algorithm above is globally stable.
\end{lemma}
\begin{proof}
Assume for contradiction that exists a hospital $h \in \H$ and distribution $\sigma \in \Delta(\D)$ the are a blocking allocation for the output of \cref{alg:global_stability}, $\pi(\mathcal{S})$.
By the argument in lemma \ref{lemma:alg_glob_term} we know that there exists no $C \in \C$ such that $supp(\sigma) = C$. Since $\sigma$ is strictly individually fair we know that for any cluster $C \in\C$, if there exists $d \in C: d\in supp(\sigma)$ then $C \subseteq \supp(\sigma)$. Denote $C^* = \argmin_{C \in \C}\set{r_h^{-1}(C) : C \subseteq supp(\sigma)}$.

We claim that $h$ and $U(C^*)$ are a blocking allocation too. The distribution $U(C^*)$ is strictly individually fair and $h$ must prefer it over any distribution over $supp(\sigma)$ since $C^*$ is its favorite cluster in $\sigma$. In lemma \ref{lemma:alg_glob_term} we showed that there are no blocking allocations that consists of a single cluster at the end of the run so this is a contradiction to the assumption.
\end{proof}

==> introduction_gal.tex <==
%% stuff for intro

Many resource allocation problems can be viewed as \emph{two-sided markets}, in which there are two sets of agents, that both have preferences over the other set. In this setup, we seek a matching: a symmetric allocation in which every member from the first set is matched to a member of the other set (ads to users, drivers to customers, hospitals to students). A well-studied desiderata for such two-sided matchings is \emph{stability} \cite{gale1962college}. A matching is stable only if it leaves no pair of agents on opposite sides of the market who are not matched to each other, but would both prefer to be. In their seminal work, \cite{gale1962college} proved that in two-sided markets a stable matching always exists and can be found efficiently using a simple procedure known as the \emph{deferred acceptance} algorithm. 

There are many instances, however, where we may seek to look beyond utility-based desiderata such as stability. Suppose, for example, that the preferences of some hospitals are discriminatory, e.g. in that given two equally-qualified doctors, they display a preference towards doctors that don't live in certain neighborhoods, or doctors without kids. In this case, a stable matching may be undesirable. This raises many natural questions: How should we formally define such ``undesirable'' allocations? Can we hope to obtain strong protections for individuals whilst satisfying a reasonable notion of stability? And from an algorithmic perspective, can we use existing algorithms for finding stable matchings, or should fairness be taken in to account? 

The emerging field of \emph{algorithmic fairness} has began to address such questions, but the focus is typically in the context of one-sided allocation problems (e.g., supervised learning). The two-sided setting is unique in that we have two sets of agents, both of which have preferences over the other side. This setting is inherently a-symmetric, and accordingly, our focus will be on guaranteeing fairness of the resulting allocation for one set of agents (e.g., some notion of fairness between the doctors), whilst still maintaining a notion of stability with the other set in mind (e.g., making sure the hospitals have an incentive to remain in the system).  Studying fairness in the context of two-sided markets is well-motivated since many of the 
the resource allocation problems captured by two-sided markets are also problems that have high-stakes for the individuals involved, but in which fairness is not the only concern. 
 
 \subsection{This work: fair and stable matchings}
 
 A fundamental prerequisite is a notion of what makes a given allocation fair. In this work, we build on the approach of \emph{individual fairness} (IF) \cite{dwork2012fairness}, which assumes the existence of a task-specific similarity metric that measures how ``similar'' two individuals are (say, whether they are equally-qualified as doctors). We would like to ensure that the eventual allocation satisfies \emph{preference-informed individual fairness} (PIIF) \cite{kim2020preference}, which roughly means that there is no envy between similar individuals (i.e., a doctor $i_1$ will not prefer the outcome that a similarly-qualified doctor $i_2$ receives).


In this work, we begin to chart the landscape of \emph{fair and stable} matchings in the context of two-sided markets. Specifically,  our contributions are:


\begin{itemize}
    \item \textbf{Extending the existing notions of stability}. As mentioned above, a fundamental step towards proving both positive and negative results regarding the compatibility between fairness and stability is to define notions of stability that provide a reasonable guarantee for the hospitals without being trivially incompatible with fairness. Thus, an important part of our work is extending the classic notion of stability to the setting in which we also care about fairness.
    
    \item \textbf{Failure of composition for standard algorithms}. Our exploration builds on an important but counter-intuitive result. We show that even when the hospitals' preferences satisfy a very strong notion of fairness (say, that they must be indifferent between two equally-qualified candidates), running the classic deferred acceptance algorithm of \cite{gale1962college} is \emph{not} guaranteed to result in a fair allocation. This can be thought of an displaying a failure of \emph{composition}: even when the inputs to an algorithm are ``fair'', the result may not be. Composition has previously been highlighted as a challenge in the context of designing fair algorithms \cite{dwork2018fairness}. This stands in stark contrast to e.g. the landscape around privacy (where \emph{differential privacy} enjoys graceful composition properties, facilitating the design of complex private algorithms using private ``building blocks''). %This means that if we hope to obtain both fairness and stability, we must consider algorithms that explicitly take fairness into account.
    
    
    %[add to related work] While earlier works highlighted composition as problematic in the context of fairness, existing examples are mostly illustrative. Our result displays a natural and popular algorithm which fails to compose nicely. 
    
    \item \textbf{Compatibility of fairness and stability given fair preferences and ``simple'' metrics}: Our main technical contribution is a strong positive  result establishing that fairness and stability are compatible, when (i) the preferences of the hospitals are fair, and (ii) we place strong assumptions on the structure of the similarity metric defining fairness. Specifically, our results hold for a class of similarity metrics that we refer to as ``proto-metrics'', in which the distances between every pair of individuals must be either zero or one. Importantly, we show that that not only do fair and stable solution exist, but they can be found efficiently: we provide natural variants of doctor-first and hospital-first deferred acceptance that are guaranteed to yield fair and stable solutions.
    
    \item \textbf{Barriers for compatibility in the general case}. A natural question is whether the assumptions that the hospitals' preferences must be fair and that the metric must be ``simple'' are necessary. We provide a partial answer by demonstrating a large class of natural algorithms (extending both GS and our variants) for which removing either assumption results in a failure to yield a fair and stable solution.
\end{itemize}



%% stuff for related work

Our work bridges between the established literature on matchings, originating in the seminal work of Gale and Shapley \cite{gale1962college}, and the emerging literature on algorithmic fairness, which seeks to formalize and mitigate discrimination in algorithmic decision-making systems \cite{barocas2016big}. The latter has focused on formalizing and studying different notions of fairness, and understanding the tensions between them and possible ``accuracy'' based desiderata \cite{chouldechova2017fair, kleinberg2016inherent, hardt2016equality}. One popular approach to quantifying unfairness are group-based definitions, in which the objective is equalize some statistic across a fixed collection of ``protected'' groups. In this work we build on a different approach, using the notion of preference-informed individual fairness \cite{kim2020preference}, which combines the individual-based fairness notion proposed in \cite{dwork2012fairness} with the notion of envy freeness from game theory \cite{foley1967resource, varian1974efficiency}. Recent work \cite{dwork2018fairness} has considered the question of composition in the context of fairness, showing that in simple toy-examples fairness may fail to compose. Our results complement their findings by demonstrating this may happen for a natural and widely popular algorithm. 

Fairness has also been studied previously in the context of two-sided matchings. \cite{gusfield1989stable} introduced the \emph{equitable stable marriage problem}, where the objective is to minimize (across stable matchings) the difference between the sum of rankings of each set over their matches. This implies avoiding unequal degrees of happiness among the two sides, and \cite{giannakopoulos2015equitable} showed an algorithm that finds such a solution. This is motivated by the fact that stable matchings are in general not unique (and their number could even be exponential \cite{knuth1997stable, thurber2002concerning}), and that the algorithm introduced by \cite{gale1962college} finds the optimal stable matching for one of the sets and the worst stable matching for the other. Our approach is inherently different in that we seek a matching that is fair within one of the sets rather than across sets. \cite{freeman2021two} studied the problem of finding an allocation that satisfies \emph{envy-freeness up to one good} (EF1), for both sets simultaneously. This is a relaxation of the classic notion of envy-freeness, that requires that any pairwise envy can be eliminated by removing a single item from the envied agent’s allocation. This formulation is similar to ours in that it tries to guarantee fairness for each set separately. However, our work is conceptually different in that our focus is on the compatibility between fairness and stability, and technically different because in the one-to-one setting that we study the EF1 objective becomes vacuous. Finally, \cite{suhr2019two} study the problem of matching drivers to passengers in ride-hailing platforms, trying to achieve equal income, and by this fair, for the drivers. We focus on a different fairness notion, that is appropriate for when the preferences of the individual are potentially diverse. 




